Micro Cold Traps on the Moon

Water ice is thought to be trapped in large permanently shadowed regions (PSRs) in the Moon's polar regions, due to their extremely low temperatures. Here, we show that many unmapped cold traps exist on small spatial scales, substantially augmenting the areas where ice may accumulate. Using theoretical models and data from the Lunar Reconnaissance Orbiter, we estimate the contribution of shadows on scales from 1 km down to 1 cm, the smallest distance over which we find cold-trapping to be effective for water ice. Approximately 10-20\% of the permanent cold trap area for water is found to be contained in these "micro cold traps," which are the most numerous cold traps on the Moon. Consideration of all spatial scales therefore substantially increases the number of cold traps over previous estimates, for a total area of ~40,000 km^2. A majority of cold traps for water ice is found at latitudes >80{\deg} because permanent shadows equatorward of 80{\deg} are typically too warm to support ice accumulation. Our results show that water trapped at the lunar poles may be more accessible as a resource for future missions than previously thought.

==> shadowfraction2.tex <==
\section{Scale Dependence of Shadow and Cold Trap Areas}

To calculate the fractional area occupied by cold traps, it is necessary to determine the functions $\alpha(l,\varphi)$ and $\tau(l,\varphi)$ from equation (\ref{eq:af}). Here, $\alpha(l,\varphi) dl$ is the fractional surface area occupied by permanent shadows having dimension $l$ to $l+dl$, $\tau$ is the fraction of these permanent shadows with maximum temperature $T_{\rm max} <$ 110~K, and $\varphi$ is the latitude.

\begin{figure}[bh!]
\centering \
\includegraphics[width=70mm]{figures/shadow_frac_NAC_pfit2.pdf}
\caption{Instantaneous shadow fraction from LROC-NAC images for a range of solar incidence angles (68\deg, 69\deg, ..., 88\deg, lighter tones representing increasing incidence angle), binned in logarithmically spaced shadow patch scales from 0.5 m to 50 km. Dashed lines represent a fit to the data.}
\label{fig:ishadow}
\end{figure}

\begin{figure*} [th]
\centering \
\includegraphics[width=70mm]{figures/shadowdist_top_v5.png}
\caption{Comparison of shadow fraction from LROC image data (points) to the model (curves). Error bars indicate the mean and standard deviations within each solar incidence angle bin, and $x_\mathrm{crater}$ is the area occupied by craters within the rough terrain.}
\label{f:shadow-fraction}
\end{figure*}

\begin{figure}[bh!]
\centering \
\includegraphics[width=70mm]{figures/shadow_alpha05.pdf}
\caption{Fraction $\alpha$ (units of m$^{-1}$) of the total surface area occupied by permanent shadows as a function of latitude $\varphi$ and length scale $l$. The model curves shown assume a crater fraction of 20\% and inter-crater plains with RMS slope $\sigma_\mathrm{s} = 5.7^\circ$}
\label{fig:alpha}
\end{figure}

First, to determine $\alpha$, we tabulated values of the fractional area of instantaneous shadow from LROC images, as described above. This shadow  fraction is then used in the integral

\begin{equation}
    M(L,\varphi) = \int_{L}^{L+\delta L} \frac{\alpha(l,\varphi)}{f(l, \varphi)} dl
\end{equation}
where $f(l,\varphi)$ is the ratio of permanent to instantaneous noontime shadow, which also may depend on length scale and latitude. Figure \ref{fig:ishadow} shows the instantaneous shadow fraction over a range of scales and incidence angles, along with our model fit: 
\begin{equation}
    \log_{10}M_\textrm{fit}(L,\varphi) = B_0 + B_1\cos\varphi + B_2\log_{10}L + B_3\cos\varphi \log_{10}L
\end{equation}
with best-fit coefficients $B_0=-4.89, B_1=-1.38, B_2=0.89, B_3=-0.57$. The model also fits the observed break in slope (Fig. \ref{fig:ishadow}) at $L_\textrm{break}$ by forcing $M(L,\varphi) = M(L_\textrm{break},\varphi)$ for all $L \le L_\textrm{break}$. From the LROC-NAC data used in this study, we find $L_\textrm{break} \approx 100$~m.

We assume that $\alpha$ is not very sensitive to small changes in $l$, i.e., we observe that shadow areas increase in proportion to logarithmic size bins. In this case, over a restricted range of $l$ from $L$ to $L + \delta L$,
\begin{equation}
    \alpha(L,\varphi) = \frac{\partial}{\partial L}(fM) \approx f(L,\varphi)\frac{M(L+\delta L,\varphi)-M(L,\varphi)}{\delta L}
    \label{eq:alpha}
\end{equation}
Figure \ref{fig:alpha} displays the resulting best-fit values of $\alpha$ for a range of solar incidence angles and three length scales. These were derived using (\ref{eq:alpha}) and the shadow data from LROC, with $f$ calculated using (\ref{eq:final}) and crater depth/diameter ratio $\gamma = 0.1$.

% We find that the PSR area fraction can be modeled using
% \begin{equation}
%     \alpha(l,\varphi) = \alpha_0(l)\Big[1-e^{-1/p\cos\varphi} \Big]^q
% \end{equation}
% with best-fit parameters $p = 3, q = 5$, constrained by the latitude-dependence of the measured shadows. At the pole, $\varphi = 90\deg$, $\alpha \rightarrow \alpha_0$, we model the PSR fraction with functions of the form
% \begin{equation}
%     \alpha_0(l) = k l^w e^{-l/L_0}
%     \label{eq:alpha0}
% \end{equation}
% Equation (\ref{eq:alpha0}) has cumulative distribution functions
% \begin{equation}
%     \textrm{CDF}_{>x} = \int_{x}^{\infty} \alpha_0(l) dl = k L_0^{w+1}\Gamma(w+1,x/L_0)
% \end{equation}
% \begin{equation}
%     \textrm{CDF}_{<x} = \int_{0}^{x} \alpha_0(l) dl = k L_0^{w+1}\Big[\Gamma(w+1) - \Gamma(w+1,x/L_0)\Big]
% \end{equation}
% where $\Gamma$ is the (upper) modified gamma function. The pre-factor $k$ provides a normalization
% \begin{equation}
%     k = \bar{f} / (L_0^{w+1}\Gamma(w+1)),
% \end{equation}
% such that
% \begin{equation}
%     \textrm{CDF}_{>0} = M(0,\infty,90\deg)\bar{f} \\
% \end{equation}
% with
% \begin{equation}
%   \bar{f} = x_\textrm{c}f_\textrm{c} + (1-x_\textrm{c})f_\textrm{p}
% \end{equation}
% where $f$ is again the ratio of permanent to instantaneous shadow, and the subscripts c and p refer to the craters and inter-crater plains, respectively.

% Using the data from LROC and also that of \citet{mazarico11}, we find best-fit empirical constants $w = -0.77$, $L_0 = 100$~km. Some resulting PSR models are shown in Figure \ref{fig:mazarico_fits}.

\begin{figure}[tbh!]
\centering \
\includegraphics[width=70mm]{figures/PSR_CDF_MazaricoFits_oa1.pdf}
\caption{Cumulative fraction of the total surface area occupied by permanent shadows with length scale $l > L$. Data points are from \citet{mazarico11}, for each polar region, $>87.5$\deg.}
\label{fig:mazarico_fits}
\end{figure}

The next step is to determine the fraction $\tau$ of these permanent shadows that are cold traps. We considered two regimes: (1) shadows large enough that conduction from warm sunlit surfaces is negligible; (2) shadows small enough to be affected by lateral heat conduction. In the first case, surface temperatures in shadows are determined by the incident radiation, which we calculate exactly. For the case of small shadows, the $\tau$ term is indeed affected by lateral heat conduction, which we estimate as follows.

\subsection{Craters}

For each latitude $\varphi$ and length scale $l$, there exists a maximum depth/diameter ratio $\gamma_\textrm{c}(l,\varphi)$ corresponding to craters whose permanently shadowed portions have $T_\textrm{max} < 110$~K. Since shallower craters have colder PSRs \citep{ingersoll92,vasavada99}, the criterion $\gamma < \gamma_\textrm{c}$ is sufficient to determine whether a PSR is a cold trap. For large $l$, $\gamma_\textrm{c} \rightarrow \gamma_\textrm{c,0}$, the value absent conduction. In determining $\gamma_\textrm{c}$ for smaller $l$, we used a 2-d heat conduction model (described below) to estimate the contribution of lateral conduction into PSRs. Figure \ref{fig:gamma} shows a summary of these results. 

% From our model results, we find that the critical depth/diameter ratio for cold-trapping craters can be described by
% \begin{equation}
%     \gamma_\textrm{c}(l,\varphi) = \gamma_\textrm{c,0}(\varphi) \bigg[1-e^{-\sqrt{l/l_\textrm{0}(\varphi)}}\bigg]
% \label{eq:gamma}
% \end{equation}
% where the characteristic length scale is
% \begin{equation}
%     l_\textrm{0}(\varphi) = \textrm{(1 cm)}\times e^{\eta \cos \varphi}   % it would be better to use m instead of cm
% \end{equation}
% with $\eta = 1/\cos\varphi_0$, with $\varphi_0 \approx$ 85.6\deg. 
The 2-d model indicates that conduction eliminates cold traps with sizes ranging from $\sim1$~cm near the pole, to $\sim10$~m at 60\deg\ latitude. We note that this size range depends on the choice of $T_\textrm{max}$ for cold-trapping, and neglects multiple-shadowing.

\begin{figure}[tbh!]
\centering \
\includegraphics[width=70mm]{figures/criticalDepthDiam_gammaC_l_lat.pdf}
\caption{Critical depth/diameter ratio $\gamma_\textrm{c}$ of craters, for which $\gamma < \gamma_\textrm{c}$ indicates the PSR is a cold trap for water ice. }
\label{fig:gamma}
\end{figure}

$\gamma_\textrm{c,0}(\varphi)$ is calculated from the analytical boundary conditions derived by \citet{ingersoll92}, coupled to the 1-d thermal model.  Using the modeled values of $\gamma_\textrm{c}$, we then calculate
\begin{equation}
    \tau_\textrm{c}(l,\varphi) = \int_{0}^{\gamma_\textrm{c}(l,\varphi)} P(\gamma)d\gamma
\end{equation}
where $P(\gamma)$ is the log-normal probability distribution function for crater depth/diameter ratio $\gamma$: 
\begin{align}
    P(\gamma; \mu, \sigma) &= \frac{1}{\gamma s \sqrt{2\pi}} e^{-\frac{(\ln \gamma - m)}{2s^2}} \\
    m &= \ln\left( \frac{\mu}{\sqrt{1+\frac{\sigma}{\mu^2}}}\right) \\
    s^2 &= \ln\left( 1 + \frac{\sigma}{\mu^2}\right)
\end{align}

Figure \ref{fig:tau} displays results of this calculation for the two log-normal probability distributions `A' (deeper craters, $\mu = 0.14$) and `B' (shallower craters, $\mu = 0.076$).

\begin{figure}[tbh!]
\centering \
\includegraphics[width=70mm]{figures/coldtrap_fraction_tau_craterAB.pdf}
\caption{Fraction of permanently shadowed regions (PSR) inside craters that are cold traps for water ice, $T_{\rm max} < 110$~K. Results are shown for two log-normal probability distributions `A' (deeper craters, $\mu = 0.14$) and `B' (shallower craters, $\mu = 0.076$). Contours are plotted for $\tau = 0.1, 0.2,...,0.9$. }
\label{fig:tau}
\end{figure}

\subsection{Rough Surface}
Although we did not explicitly model lateral conduction for the Gaussian rough surface, our model results absent conduction provide an upper limit on the relative cold-trapping area, which we call $\tau_\textrm{p,0}(\sigma_\textrm{s};\varphi)$. This quantity (the ratio of cold-trap area to PSR area, absent conduction) is scale-independent, but instead depends on the RMS slope, $\sigma_\textrm{s}$. We modeled the latitude- and scale-dependence of lateral conduction assuming it is the same for rough surfaces as for craters.

\subsection{Distribution Functions}

A number of useful measures of cold trap and PSR area can be determined once $\alpha$ and $\tau$ are determined. Defining the fractional cold trap area, per unit length,
\begin{equation}
    A_l \equiv \frac{\partial A(\varphi,l)}{\partial l} = \alpha(\varphi,l)\tau(\varphi,l)
\end{equation}
and
\begin{equation}
    A_{l\varphi} \equiv \frac{\partial^2 A(\varphi,l)}{dl d\varphi} = \alpha(\varphi,l)\tau(\varphi,l)\cos\varphi
\end{equation}
For each latitude $\varphi$, the fractional area of cold traps with dimensions from $L$ to $L'$ is
\begin{equation}
    A(L,L',\varphi) = \int_L^{L'} A_{l} dl
\end{equation}
and the total fractional area of these cold traps for the whole hemisphere is
\begin{align}
    A(L,L') &= \int_0^{\pi/2} \int_L^{L'} A_{l\varphi} dl d\varphi \\ 
    &= \int_0^{\pi/2} \int_L^{L'} \alpha(\varphi,l)\tau(\varphi,l)\cos \varphi dl d\varphi
\end{align}
The cumulative distribution function is:
\begin{equation}
    \textrm{CDF}_{<x} = A(0,x) = \int_0^{\pi/2} \int_0^x A_{l\varphi}dld\varphi
\end{equation}
The number of cold traps from $L$ to $L'$ per unit area at a given latitude is
\begin{equation}
    N(L,L',\varphi) = \int_L^{L'} A_l l^{-2} dl
\end{equation}
and the number per unit area over the hemisphere is
\begin{equation}
    N(L,L') = \int_0^{\pi/2} \int_L^{L'} A_{l\varphi} l^{-2} dl d\varphi
\end{equation}
The number of PSRs per unit area is
\begin{equation}
    N_\textrm{PSR}(L,L') = \int_0^{\pi/2} \int_L^{L'} \alpha(\varphi,l)\cos\varphi~l^{-2}  dl d\varphi
\end{equation}
Over latitudes 0 to 90$^\circ$, the total volume per unit area of hemispherical cold traps with dimensions from $L$ to $L'$ is
\begin{align}
    V(L,L') &= \frac{1}{3}\int_0^{\pi/2} \int_L^{L'} A_{l\varphi}l dl d\varphi\\
    &= \frac{1}{3}\int_0^{\pi/2} \int_L^{L'} N(l) l^3 dl d\varphi
\end{align}
where $N(L) = N(L,L+\delta)$ in the limit $\delta \rightarrow 0$.

% with analogy to equation (\ref{eq:gamma}) we have
% \begin{equation}
%     \tau_\textrm{p}(\sigma_\textrm{s};l,\varphi) = \tau_\textrm{p,0}(\sigma_\textrm{s};\varphi) \bigg[1-e^{-\sqrt{l/l_\textrm{0}(\varphi)}}\bigg]
% \end{equation}


